Self-Supervised CSF Inpainting with Synthetic Atrophy for Improved Accuracy Validation of Cortical Surface Analyses

Accuracy validation of cortical thickness measurement is a difficult problem due to the lack of ground truth data. To address this need, many methods have been developed to synthetically induce gray matter (GM) atrophy in an MRI via deformable registration, creating a set of images with known changes in cortical thickness. However, these methods often cause blurring in atrophied regions, and cannot simulate realistic atrophy within deep sulci where cerebrospinal fluid (CSF) is obscured or absent. In this paper, we present a solution using a self-supervised inpainting model to generate CSF in these regions and create images with more plausible GM/CSF boundaries. Specifically, we introduce a novel, 3D GAN model that incorporates patch-based dropout training, edge map priors, and sinusoidal positional encoding, all of which are established methods previously limited to 2D domains. We show that our framework significantly improves the quality of the resulting synthetic images and is adaptable to unseen data with fine-tuning. We also demonstrate that our resulting dataset can be employed for accuracy validation of cortical segmentation and thickness measurement.

==> table2_FLAIR.tex <==
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\begin{table}[t]
\centering

% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
\begin{tabular}{C{0.55in}|C{0.55in}|C{0.6in} C{0.25in} C{0.25in} C{0.6in} C{0.75in}|C{0.3in}|C{0.3in}|C{0.3in}}
\hline
    \multicolumn{7}{c}{\textbf{Validation Experiment}} & \multicolumn{3}{|c}{\textbf{FL Model}} \\
\hline
\hline
    \multirow{2}{0.55in}{} & \multirow{2}{0.55in}{} & \multicolumn{5}{c|}{ Input Channels} & \multirow{2}{0.3in}{\tiny L1 \newline $\downarrow$} & \multirow{2}{0.3in}{\tiny PSNR \newline $\uparrow$} & \multirow{2}{0.3in}{\tiny SSIM \newline $\uparrow$} \\
    \cline{3-7}
    & & \tiny $\phi(\mathbf{I}_{FL},\mathbf{M}_{\text{dr}})$ & \tiny $\mathbf{M}_{\text{tis}}$ & \tiny $\mathbf{I}_{\text{tis}}$ & \tiny $\phi(\mathbf{I}_{T1},\mathbf{M}_{\text{dr}})$ & \tiny $\mathbf{E}(\phi(\mathbf{I}_{FL},\mathbf{M}_{\text{dr}}))$ & & & \\
\hline 
    \rowcolor{Thistle1}
    & \tiny 3D CNN & \tiny\checkmark & \tiny\checkmark & & & & \tiny 9.13 & \tiny 25.65 & \tiny 0.66 \\ 
    \rowcolor{Thistle2}
    \cellcolor{Thistle1} & \tiny 3D CNN & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & & & \tiny 8.73 & \tiny 26.52 & \tiny 0.70 \\
    \rowcolor{Thistle1}
    & \tiny 3D CNN & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & &  \tiny 7.98 & \tiny 25.71 & \tiny 0.68 \\
    \rowcolor{Thistle2}
    \multirow{-4}{0.55in}{\cellcolor{Thistle1}\tiny Input channel ablation} & \tiny 3D CNN & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & & \tiny\checkmark & \tiny 8.01 & \tiny 25.80 & \tiny 0.71 \\    
\hline
    \rowcolor{Khaki1}
     \tiny no SPE & \tiny 3D CNN & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny 9.33 & \tiny 24.42 & \tiny 0.68 \\ 
\hline
    \rowcolor{LightBlue1}
    & \tiny 3D CNN & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny 4.19 & \tiny 21.82 & \tiny 0.74 \\
    \rowcolor{LightBlue2}
    \cellcolor{LightBlue1} & \tiny 2.5D CNN & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny3.43 & \tiny 22.24 & \tiny 0.75 \\ 
    \rowcolor{LightBlue1}
    & \tiny 2D LaMA & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny  2.51 &\tiny 28.97 &\tiny 0.89 \\ 
    \rowcolor{LightBlue2}
    \multirow{-4}{0.55in}{\cellcolor{LightBlue1} \tiny Generator architectures} & \tiny 2.5D LaMA & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \tiny \textbf{1.17} & \tiny\textbf{32.41} & \tiny\textbf{0.91} \\ 
    \hline
    \rowcolor{DarkSeaGreen1}
    \tiny Ours & \tiny 3D CNN & \tiny\checkmark & \tiny\checkmark & \tiny\checkmark & \checkmark & \tiny\checkmark &\tiny 6.63 &\tiny 27.80 & \tiny0.81 \\ 
 \hline
\end{tabular}
\caption{\yyy{Quantitative results for ground truth validation studies with FLAIR images.}}
\label{tab:quantitativeMetrics_FLAIR}
\end{table}
